Effectiveness of Pre-training for Few-shot Intent Classification

This paper investigates the effectiveness of pre-training for few-shot intent classification. While existing paradigms commonly further pre-train language models such as BERT on a vast amount of unlabeled corpus, we find it highly effective and efficient to simply fine-tune BERT with a small set of labeled utterances from public datasets. Specifically, fine-tuning BERT with roughly 1,000 labeled data yields a pre-trained model -- IntentBERT, which can easily surpass the performance of existing pre-trained models for few-shot intent classification on novel domains with very different semantics. The high effectiveness of IntentBERT confirms the feasibility and practicality of few-shot intent detection, and its high generalization ability across different domains suggests that intent classification tasks may share a similar underlying structure, which can be efficiently learned from a small set of labeled data. The source code can be found at https://github.com/hdzhang-code/IntentBERT.

==> figures/figure_ablation_study.tex <==
\begin{figure}[H]
     \centering
     \includegraphics[scale = 0.25]{resources/ablation_study.png}
\caption{Ablation study. BANK here denotes BANKING77. $\rightarrow$ represents moving to the next stage, and $+$ stands for joint training. All the experiments are evaluated from 5-way, 2-shot tasks}
\label{figure: ablation study}
\end{figure}

==> tables/related.tex <==
\section{Related Works}
\subsection{Few-shot Intent Detection}
There are some recent attempts that adapt these ideas to intent detection.

RobustTC \cite{NAACL18} develops dynamic metrics by clustering similar tasks into groups.

Induction network \cite{geng2019few} produces better representations for intents via dynamic routing.

\citet{xia2020composed, xia2020cg} generate novel utterances to augment the annotated data set. 

\citet{nguyen2020dynamic} design elaborate metric function to compare utterances. 

\citet{zhang2020discriminative} propose to warm up BERT-based model by NLI (Natural Language Inference) task.

\cite{dopierre2020few} devise a clustering algorithm to tag pseudo-label on unlabeled data, which is used to train a better model. 

\cite{zhang2020intent} exploits WikiHow to construct a supervised dataset to further train langugage model such as RoBERTa for intent detection.

\cite{yu2021few} employs BERT to encode the utterances and dot-product to measure the utterance similarity.

There are several works focusing on other scenarios, including \cite{hou2020few} on multi-label intent detection, \cite{bhathiya2020meta} on joint intent detection and slot filling. 

It is noted that current works employ distinctive evaluation settings, rendering fair comparison difficult, and thus make it difficult to learn what the real status the current research is.



However, these works do not address the domain shift and adaptation to a new domain.

==> tables/table_mainResult.tex <==
\begin{table*}[t]
%% local redefinitions
% \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
% \renewrobustcmd{\boldmath}{}
\centering
\small
\begin{tabular}{lccccccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & 
\multicolumn{1}{c}{\multirow{2}{*}{$\mathcal{D}_{\text{target}}^{\text{unlabeled}}$}} & 
\multicolumn{2}{c}{BANKING77}  &
\multicolumn{2}{c}{MCID}    &
\multicolumn{2}{c}{HINT3}  
\\
\cmidrule(lr){3-4}  \cmidrule(lr){5-6}  \cmidrule(lr){7-8}
& & 2-shot  & 10-shot  & 2-shot & 10-shot & 2-shot & 10-shot  \\
\midrule
BERT-Freeze & \xmark & 52.6\tiny{$~\pm$12.4} & 70.0\tiny{$~\pm$11.7} & 57.8\tiny{$~\pm$11.7} & 72.4\tiny{$~\pm$10.7} & 47.3\tiny{$~\pm$12.1} & 66.8\tiny{$~\pm$10.5} \\
BERT-MLM & \cmark &  \textbf{80.5\tiny{$~\pm$11.1}}  & \textbf{90.1\tiny{$~\pm$7.8}}  &  63.0\tiny{$~\pm$12.4}  &  75.5\tiny{$~\pm$10.4}  &  72.0\tiny{$~\pm$11.9}  &   85.6\tiny{$~\pm$8.8}  \\
% CONVBERT~\cite{mehri2020dialoglue} & \xmark & 68.3\tiny{$~\pm$12.3} & 86.6\tiny{$~\pm$8.2} & 67.7\tiny{$~\pm$11.5} & 83.5\tiny{$~\pm$7.9} & 72.6\tiny{$~\pm$10.9} & 87.2\tiny{$~\pm$7.9} \\
CONVBERT & \xmark & 68.3\tiny{$~\pm$12.3} & 86.6\tiny{$~\pm$8.2} & 67.7\tiny{$~\pm$11.5} & 83.5\tiny{$~\pm$7.9} & 72.6\tiny{$~\pm$10.9} & 87.2\tiny{$~\pm$7.9} \\
% TOD-BERT~\cite{wu2020tod} & \xmark & 77.7\tiny{$~\pm$7.4} & 89.4 \tiny{$~\pm$5.1} &  64.1\tiny{$~\pm$9.0}  & 77.7\tiny{$~\pm$11.0} &  68.9\tiny{$~\pm$11.7} &  83.5\tiny{$~\pm$8.6}  \\
TOD-BERT & \xmark & 77.7\tiny{$~\pm$7.4} & 89.4 \tiny{$~\pm$5.1} &  64.1\tiny{$~\pm$9.0}  & 77.7\tiny{$~\pm$11.0} &  68.9\tiny{$~\pm$11.7} &  83.5\tiny{$~\pm$8.6}  \\
% USE-ConveRT$\ssymbol{5}$~\cite{casanueva2020efficient} & \xmark  & -- & 85.2 & -- & -- & -- & -- \\
USE-ConveRT$\ssymbol{5}$ & \xmark  & -- & 85.2 & -- & -- & -- & -- \\
% DNNC~\cite{zhang2020discriminative} & \xmark   & 67.5\tiny{$~\pm$15.4} & 89.8\tiny{$~\pm$7.5} & 56.2\tiny{$~\pm$16.7} & 80.0\tiny{$~\pm$9.9} & 64.1\tiny{$~\pm$14.8} & 87.9\tiny{$~\pm$8.1}
DNNC & \xmark   & 67.5\tiny{$~\pm$15.4} & 89.8\tiny{$~\pm$7.5} & 56.2\tiny{$~\pm$16.7} & 80.0\tiny{$~\pm$9.9} & 64.1\tiny{$~\pm$14.8} & 87.9\tiny{$~\pm$8.1}
\\
% WikiHowRoBERTa~\cite{zhang2020intent} & \xmark  & 34.9\tiny{$~\pm$10.5} & 41.6\tiny{$~\pm$10.1} & 30.8\tiny{$~\pm$9.9} & 36.4\tiny{$~\pm$9.7} & 31.7\tiny{$~\pm$10.3} & 39.0\tiny{$~\pm$9.9}
WikiHowRoBERTa & \xmark  & 34.9\tiny{$~\pm$10.5} & 41.6\tiny{$~\pm$10.1} & 30.8\tiny{$~\pm$9.9} & 36.4\tiny{$~\pm$9.7} & 31.7\tiny{$~\pm$10.3} & 39.0\tiny{$~\pm$9.9}
\\
\midrule
IntentBERT (HWU64) & \xmark  & 78.4\tiny{$~\pm$10.6}  & 90.0\tiny{$~\pm$7.5}  & \textbf{74.5\tiny{$~\pm$11.9}}  & \textbf{85.9\tiny{$~\pm$8.8}}  & \textbf{77.9\tiny{$~\pm$10.6}}  & \textbf{89.4\tiny{$~\pm$7.9}} \\
IntentBERT (OOS) & \xmark  & \textbf{82.4\tiny{$~\pm$8.3}} & \textbf{91.8\tiny{$~\pm$4.2}}  & \textbf{77.1\tiny{$~\pm$9.0}} & \textbf{88.1\tiny{$~\pm$5.9}}  & \textbf{80.1\tiny{$~\pm$10.4}} & \textbf{90.2\tiny{$~\pm$7.4}}  \\
IntentBERT (OOS)+MLM & \cmark  & \textbf{88.9\tiny{$~\pm$9.0}} & \textbf{95.2\tiny{$~\pm$5.1}}  & \textbf{86.3\tiny{$~\pm$9.8}} & \textbf{92.4\tiny{$~\pm$6.2}}  &  \textbf{87.1\tiny{$~\pm$9.8}} & \textbf{94.0\tiny{$~\pm$6.0}} \\
\bottomrule
\end{tabular}
% \caption{Main results for $5$-way tasks. $\ssymbol{5}$ stands for results from the original paper. $\ssymbol{2}$ represents models that employ Roberta.}
\caption{Main results for $5$-way tasks. $\ssymbol{5}$ stands for results from the original paper.}
\label{table: main result, effectiveness of our methods}
\end{table*}

==> tables/table_mainResult_backup.tex <==
\begin{table*}[t]
%% local redefinitions
% \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
% \renewrobustcmd{\boldmath}{}
\centering
\small
\begin{tabular}{lccccccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & 
\multicolumn{1}{c}{\multirow{2}{*}{$\mathcal{D}_{\text{target}}^{\text{unlabeled}}$}} & 
\multicolumn{2}{c}{BANKING77}  &
\multicolumn{2}{c}{MCID}    &
\multicolumn{2}{c}{HINT3}  
\\
\cmidrule(lr){3-4}  \cmidrule(lr){5-6}  \cmidrule(lr){7-8}
& & 2-shot  & 10-shot  & 2-shot & 10-shot & 2-shot & 10-shot  \\
\midrule
BERT-Freeze & \xmark & 52.6\tiny{$~\pm$12.4} & 70.0\tiny{$~\pm$11.7} & 57.8\tiny{$~\pm$11.7} & 72.4\tiny{$~\pm$10.7} & 47.3\tiny{$~\pm$12.1} & 66.8\tiny{$~\pm$10.5} \\
BERT-MLM & \cmark &  80.5\tiny{$~\pm$11.1}  & 90.1\tiny{$~\pm$7.8}  &  63.0\tiny{$~\pm$12.4}  &  75.5\tiny{$~\pm$10.4}  &  72.0\tiny{$~\pm$11.9}  &   85.6\tiny{$~\pm$8.8}  \\
CONVBERT~\cite{mehri2020dialoglue} & \xmark & 68.3\tiny{$~\pm$12.3} & 86.6\tiny{$~\pm$8.2} & 67.7\tiny{$~\pm$11.5} & 83.5\tiny{$~\pm$7.9} & 72.6\tiny{$~\pm$10.9} & 87.2\tiny{$~\pm$7.9} \\
TOD-BERT~\cite{wu2020tod} & \xmark & 77.7\tiny{$~\pm$7.4} & 89.4 \tiny{$~\pm$5.1} &  64.1\tiny{$~\pm$9.0}  & 77.7\tiny{$~\pm$11.0} &  68.9\tiny{$~\pm$11.7} &  83.5\tiny{$~\pm$8.6}  \\
USE-ConveRT$\ssymbol{5}$~\cite{casanueva2020efficient} & \xmark & -- & 85.2 & -- & -- & -- & -- \\
DNNC~\cite{zhang2020discriminative}  & \xmark & 67.5\tiny{$~\pm$15.4} & 89.8\tiny{$~\pm$7.5} & 56.2\tiny{$~\pm$16.7} & 80.0\tiny{$~\pm$9.9} & 64.1\tiny{$~\pm$14.8} & 87.9\tiny{$~\pm$8.1} \\
WikiHowRoBERTa~\cite{zhang2020intent}  & \xmark & 34.9\tiny{$~\pm$10.5} & 41.6\tiny{$~\pm$10.1} & 30.8\tiny{$~\pm$9.9} & 36.4\tiny{$~\pm$9.7} & 31.7\tiny{$~\pm$10.3} & 39.0\tiny{$~\pm$9.9} \\
\midrule
IntentBERT (HWU64) & \xmark & \textbf{78.4\tiny{$~\pm$10.6}}  & \textbf{90.0\tiny{$~\pm$7.5}}  & \textbf{74.5\tiny{$~\pm$11.9}}  & \textbf{85.9\tiny{$~\pm$8.8}}  & \textbf{77.9\tiny{$~\pm$10.6}}  & \textbf{89.4\tiny{$~\pm$7.9}} \\
IntentBERT (OOS) & \xmark & \textbf{82.4\tiny{$~\pm$8.3}} & \textbf{91.8\tiny{$~\pm$4.2}}  & \textbf{77.1\tiny{$~\pm$9.0}} & \textbf{88.1\tiny{$~\pm$5.9}} & \textbf{80.1\tiny{$~\pm$10.4}} & \textbf{90.2\tiny{$~\pm$7.4}}  \\
IntentBERT (OOS)+MLM & \cmark & \textbf{88.9\tiny{$~\pm$9.0}} & \textbf{95.2\tiny{$~\pm$5.1}}  & \textbf{86.3\tiny{$~\pm$9.8}} & \textbf{92.4\tiny{$~\pm$6.2}} &  \textbf{87.1\tiny{$~\pm$9.8}} & \textbf{94.0\tiny{$~\pm$6.0}} \\
\bottomrule
\end{tabular}
% \caption{Main results for $5$-way tasks. $\ssymbol{5}$ stands for results from the original paper. $\ssymbol{2}$ represents models that employ Roberta.}
\caption{Main results for $5$-way tasks. $\ssymbol{5}$ stands for results from the original paper.}
\label{table: main result, effectiveness of our methods}
\end{table*}
